Toward Better Generalization Bounds with Locally Elastic Stability

Algorithmic stability is a key characteristic to ensure the generalization ability of a learning algorithm. Among different notions of stability, \emph{uniform stability} is arguably the most popular one, which yields exponential generalization bounds. However, uniform stability only considers the worst-case loss change (or so-called sensitivity) by removing a single data point, which is distribution-independent and therefore undesirable. There are many cases that the worst-case sensitivity of the loss is much larger than the average sensitivity taken over the single data point that is removed, especially in some advanced models such as random feature models or neural networks. Many previous works try to mitigate the distribution independent issue by proposing weaker notions of stability, however, they either only yield polynomial bounds or the bounds derived do not vanish as sample size goes to infinity. Given that, we propose \emph{locally elastic stability} as a weaker and distribution-dependent stability notion, which still yields exponential generalization bounds. We further demonstrate that locally elastic stability implies tighter generalization bounds than those derived based on uniform stability in many situations by revisiting the examples of bounded support vector machines, regularized least square regressions, and stochastic gradient descent.

==> old-intro.tex <==
\section{Introduction}
\label{sec:introduction}

%\swj{be careful about terminologies: sensitivity, difference, etc. class membership}

A central question in machine learning is how the performance of an algorithm on the training set carries over to unseen data. Continued efforts to address this question have given rise to numerous generalization error bounds on the gap between the population risk and empirical risk, using a variety of approaches from statistical learning theory \citep{vapnik1979estimation,vapnik2013nature,bartlett2002rademacher,bousquet2002stability}. Among these developments, algorithmic stability stands out as a general approach that allows one to relate certain specific properties of an algorithm to its generalization ability. Loosely speaking, \cite{bousquet2002stability} show that an algorithm would generalize well on new data if this algorithm is uniformly stable in the sense that its loss function does not change much with respect to a small perturbation in the training set.

%When turning their focus to deep neural networks, 
When it comes to deep neural networks, however, many existing approaches in statistical learning theory stop short of providing meaningful generalization bounds. These bounds can, for example, be too loose to be useful from a practical standpoint or, worse, even increase with the size of the training set~\citep{nagarajan2019uniform}. In brief, the incapabilities of these approaches are largely due to the highly \textit{nonconvex} nature of the commonly used loss functions in deep learning. Concerning algorithmic stability, in particular, this nonconvexity leads to a substantial \textit{worst-case} change in the value of the loss functions with a small perturbation of the input. As a concrete example, while uniform stability hardly depends on the label information of the training set, the generalization ability of neural networks is contingent upon whether the labels are true or corrupted. Explicitly, the generalization error would be small with true labels, and large with random labels due to memorization. This reality has motivated \cite{zhang2016understanding}, among others, to raise the following pressing question: 
\begin{center}
\textit{Can we develop a weaker stability notion that is tailor-made\\ for deep neural networks for better generalization bounds?}
\end{center}
\begin{figure*}[t]
		\centering
		 \subfigure[Sensitivity of neural networks.]{
			\centering
			\includegraphics[scale=0.4]{Figs/test_train_absolute_influence_100_100.png}
			\label{fig:NNs-IF}}
        \subfigure[Sensitivity of a linear model.]{
			\centering
			\includegraphics[scale=0.4]{Figs/test_train_absolute_influence_linear_100_100_60_1e-07.png}
			\label{fig:Linear-IF}}
		\caption{Class-level sensitivity approximated by influence functions for an 18-layer ResNet and a linear model on CIFAR-10. The vertical axis denotes the classes in the test data and the horizontal  axis denotes the classes in the training data. The class-level sensitivity from class $a$ in the training data to class $b$ in the test data is defined as $C(c_a, c_b) = \frac{1}{|S_a| \times |\tilde{S}_b|}\sum_{z_i \in S_a} \sum_{z \in \tilde{S}_b}|l(\hat{\theta},z)-l(\hat{\theta}^{\backslash i},z)|$, where $S_a$ denotes the set of examples from class $a$ in the training data and $\tilde{S}_b$ denotes set of examples from class $b$ in the test data. More details are in Appendix \ref{sec:experiments}.
		}
		\label{fig:IF-results}
\end{figure*}
To tackle this question, in this paper we begin with several observations from Figure~\ref{fig:IF-results}. The left panel reveals that the sensitivity of neural networks is highly contingent upon the label information. To be precise, consider training two models on the CIFAR-10 dataset \citep{krizhevsky2009learning} and another dataset obtained by removing one training example, say an image of a plane, from CIFAR-10, respectively. Figure~\ref{fig:IF-results} shows that the difference between the loss function values for the two models \textit{depends} on the label of the test image that the loss function is evaluated at: the difference between the loss function values, or sensitivity for short, is significant if the test image is another plane, and the sensitivity is small if the test image is from a different class, such as car or cat. Concretely, the average plane-to-plane difference is about seven times the average plane-to-cat difference. The dependence on whether the two images belong to the same class results
in a pronounced diagonal structure in Figure~\ref{fig:NNs-IF}, which is consistent with an earlier finding in \cite{he2020local}. In particular, this structural property of the loss function differences clearly demonstrates that uniform stability fails to capture how sensitive the loss function is in the
\textit{population} sense for neural networks. In 
%stark 
contrast, linear models do not exhibit such a strong dependence on the class of images, as evidenced by the absence of a diagonal structure in Figure~\ref{fig:Linear-IF}. 
%\swj{do we have experiments with other models such as SVM?}. 
Taken together, these two plots suggest a distinctive characteristic of deep neural networks compared to linear classifiers.


Motivated by this crucial property of deep neural networks, this paper makes a two-fold contribution toward understanding the generalization ability of modern neural networks. As our \textbf{first contribution}, we introduce a new notion of algorithmic stability that is referred to as \textit{locally elastic stability} to take into account the message conveyed by Figure~\ref{fig:IF-results}. This new stability notion imposes a data-dependent bound on the sensitivity of the loss function, as opposed to a constant bound that uniform stability and many of its relaxations use. Taking the example of the CIFAR-10 dataset, locally elastic stability defines its sensitivity bound as a bivariate function taking as input any pair of images. The sensitivity bound evaluated on (plane, cat), for instance, offers a (tight) bound on the change of the loss function evaluated at \textit{any} cat image, due to the removal of \textit{any} plane image from the training set.

%for comparison, locally elastic stability is defined as a sensitivity bound that is in effect a bivariate function taking as input any pair of images. We often require the sensitivity bound to depend on the images only through their classes. 
%%the form $(\text{class}_1, \text{class}_2)$ from the 10 classes in CIFAR-10, such as (plane, cat), while the earlier stability-based approach uses a uniform bound on all 100 pairs of classes. 

The \textbf{second contribution} of this paper is to develop a generalization bound for any locally elastically stable
algorithms. This new generalization bound is obtained by a fine-grained analysis of the empirical risk using the McDiarmid inequality. More specifically, our results show that the generalization error is, loosely speaking, upper bounded by the expectation of the sensitivity function associated with locally elastic stability over the population of training examples. Assuming uniform stability, however, classical generalization bounds are mainly determined by the worst possible sensitivity over all pairs of training examples. 
As a consequence, our bound is tighter than that given by uniform stability if the loss function sensitivity is largely captured by the classes of the two images, just as in the case of neural networks. Otherwise, to be complete, we remark that the new generalization bound might not improve as much, for example, in the case of linear classifiers. This perhaps explains why locally elastic stability as such an intuitive extension of uniform stability has never been considered in the vast literature.


% evaluated at an image of plane for the neural networks trained on the CIFAR-10 dataset and the loss function 
%%In words, for all training sets S, and all training points in S (not including z), the worst possible difference (using all possible z) between the loss function evaluated at z for the function obtained using training set S and the loss function evaluated at z for the function obtained using the new training set S i,z will be at most β. This β is typically itself a function of n [2].
% \textit{Hardt et al. (2016) give an upper bound on the generalization error of a model trained with stochastic
% gradient descent in terms of the number of steps gradient descent took. Their analysis goes through
% the notion of uniform stability (Bousquet \& Elisseeff, 2002). As we point out in this work, uniform
% stability of a learning algorithm is independent of the labeling of the training data. Hence, the
% concept is not strong enough to distinguish between the models trained on the true labels (small
% generalization error) and models trained on random labels (high generalization error). This also
% highlights why the analysis of Hardt et al. (2016) for non-convex optimization was rather pessimistic,
% allowing only a very few passes over the data. Our results show that even empirically training neural
% networks is not uniformly stable for many passes over the data. Consequently, a weaker stability
% notion is necessary to make further progress along this direction.}

%%\zhun{put two good images here as Motivating Examples}
% \paragraph{Our contributions.}

% \paragraph{Outline of the paper.}

\subsection{Related Work}


\iffalse
Geometric properties of DNNs:
\begin{itemize}
    \item class/cross-class property: local elasticity\citep{he2020local}, stiffness \citep{fort2019stiffness}, neural collapse \citep{papyan2020prevalence}, class/cross-class structure \citep{papyan2020traces}
    \item Data structure: long-tail distribution\citep{zhu2014capturing}, long tail theory \citep{feldman2020does}, long-tail verification \citep{feldman2020neural}; the hidden manifold model for data structure \citep{goldt2019modelling}
\end{itemize}
\fi

%Stability papers: 



%\begin{itemize}
    %\item general stability: stability and generalization %\citep{bousquet2002stability}, Generalization bounds for uniformly stable algorithm \citep{feldman2018generalization}, High probability %generalization bounds for uniformly stable algorithms with nearly optimal rate\citep{feldman2019high}, A Second-order Look at Stability and Generalization \citep{maurer2017second},  Sharper Bounds for Uniformly Stable Algorithms \citep{bousquet2020sharper}, Average Stability is Invariant to Data Preconditioning. Implications to Exp-concave Empirical Risk Minimization \citep{gonen2017average}, Learnability, stability and uniform convergence \citep{shalev2010learnability}, Learning theory: stability is sufficient for generalization and necessary and sufficient for consistency of empirical risk minimization \citep{mukherjee2006learning}, Almost-everywhere algorithmic stability and generalization error \citep{kutin2002almost}
    
   % \item stability for SGD: stability of SGD \citep{hardt2016train}, Data-Dependent Stability of Stochastic Gradient Descent \citep{kuzborskij2018data}, Stability of Stochastic Gradient Descent on Nonsmooth Convex Losses \citep{bassily2020stability}, Fine-Grained Analysis of Stability and Generalization for Stochastic Gradient Descent \citep{lei2020fine}, High probability convergence and uniform stability bounds for nonconvex stochastic gradient descent \citep{madden2020high} 
%\end{itemize}

\paragraph{Algorithmic Stability.} Ever since \citet{kearns1999algorithmic} and \citet{bousquet2002stability} propose the notions of uniform stability and hypothesis stability, a copious line of works has been devoted to extending and elaborating on their frameworks. In \citet{mukherjee2006learning}, \citet{shalev2010learnability} and \citet{kutin2002almost}, the authors show there exist cases where stability is the key necessary and sufficient condition for learnability but uniform convergence is not.
On one hand, error stability is not strong enough to guarantee generalization \citep{kutin2012almost}. On the other hand, hypothesis stability guarantees generalization but only provides polynomial tail bounds. Fortunately, uniform stability guarantees generalization and further provides exponential tail bounds. In \citet{feldman2018generalization}, the authors develop the generalization bound for the cases where uniform stability parameter is of order $\Omega(1/\sqrt{m})$, 
where $m$ is the sample size. In subsequent work, \citet{feldman2019high} prove a nearly tight high probability bound for any uniformly stable algorithm. In \cite{bousquet2020sharper}, the authors provide sharper bounds than \citet{feldman2019high} and also provide general lower bounds which can be applied to certain generalized concentration inequalities. There are also works seeking to relax uniform stability such as \cite{abou2019exponential}, but their bound still has a small term that would not vanish even with an infinite sample size and a vanishing stability parameter.


In addition, researchers demonstrate that many popular optimization methods, such as stochastic gradient descent (SGD), satisfy algorithmic stability. In \citet{hardt2015train}, the authors show that SGD satisfies uniform stability. \citet{lei2020fine} further relax the smoothness and convexity assumptions, and others instead discuss the nonconvex case for SGD in more detail~\citep{kuzborskij2018data, madden2020high}.  \citet{kuzborskij2018data} recently propose another notion of data-dependent stability for SGD. Our work can be viewed as a relaxation of uniform stability and SGD will be shown to satisfy our new notion of algorithmic stability. 
 
 \paragraph{Geometric Properties of Neural Networks.} There has been a line of work probing the geometric properties of neural networks. As pointed in \cite{zdeborova2020understanding}, building theory of deep learning may require an understanding of the intrinsic interplay between the architecture of the neural network, the behavior of the algorithm used for learning and the structure in the data. On one hand, the influence of data structure on learning neural networks is analyzed. For example, \cite{he2020local} recently introduce a phenomenon termed local elasticity in training neural networks, implying that the interaction between two examples is heavily contingent upon whether their labels are the same or not. Similarly, \cite{fort2019stiffness} propose the stiffness depending on the class membership to illustrate the generalization of neural networks. Furthermore, the dynamics of within-class and cross-class structures is analyzed in \cite{papyan2020traces} and \cite{papyan2020prevalence}. On the other hand, different mathematical models are proposed to model the structure of real-world data, such as the long tail theory \citep{zhu2014capturing, feldman2020does, feldman2020neural}, and the hidden manifold model \citep{goldt2019modelling}. Lately, \citet{yu2020learning} unveil several profound geometric properties of neural networks in the feature space from the viewpoint of discriminative representations (see also \citet{papyan2020prevalence,anonymous2021deep}).
 
 %This paper moves further to derive a better generalization bound with the help of these geometric properties of DNNs.
